MARC: Memory-Augmented RL Token Compression for Efficient Video Understanding

The rapid progress of large language models (LLMs) has laid the foundation for multimodal models. However, visual language models (VLMs) still face heavy computational costs when extended from images to videos due to high frame rates and long durations. Token compression is a promising solution, yet most existing training-free methods cause information loss and performance degradation. To overcome this, we propose \textbf{Memory-Augmented Reinforcement Learning-based Token Compression (MARC)}, which integrates structured retrieval and RL-based distillation. MARC adopts a \textit{retrieve-then-compress} strategy using a \textbf{Visual Memory Retriever (VMR)} to select key clips and a \textbf{Compression Group Relative Policy Optimization (C-GRPO)} framework to distil reasoning ability from a teacher to a student model. Experiments on six video benchmarks show that MARC achieves near-baseline accuracy using only one frame's tokens -- reducing visual tokens by \textbf{95\%}, GPU memory by \textbf{72\%}, and latency by \textbf{23.9\%}. This demonstrates its potential for efficient, real-time video understanding in resource-constrained settings such as video QA, surveillance, and autonomous driving.

==> framework2.tex <==
\begin{figure}[t!]
    \centering
        \includegraphics[width=0.9\textwidth]{iclr2026/framework_stage2.pdf}
\caption{\textbf{Overview of Compression Group Relative Policy Optimization (C-GRPO)}. 
Here, \textbf{O} denotes the outputs from different groups, \textbf{R} the corresponding rewards, and \textbf{A} the normalized advantages. 
A compression reward $r_c$ is introduced to encourage compressed inputs to retain the reasoning ability of the uncompressed teacher model.}
    \label{fig:pipeline2}
\end{figure}

==> iclr2026/experiments.tex <==


\section{Experiments}
\label{sec:experiments}
\subsection{Experiment settings}
\label{sec:experiments_settings}


\textbf{Benchmarks.}  
To evaluate the effectiveness of our method, we conduct experiments on a suite of six widely used benchmarks: VSI-Bench \citep{yang2025thinking}, VideoMMMU~\citep{hu2025video}, MMVU~\citep{zhao2025mmvu}, MVBench~\citep{li2024mvbench}, TempCompass~\citep{liu2024tempcompass}, and VideoMME~\citep{fu2025video}. 
Figure~\ref{fig:evaluation_dataset} illustrates the evaluation benchmarks, showing the distribution based on the number of QA samples in each dataset.  


\textbf{Implementation details.} For all benchmark evaluations, videos are first uniformly sampled at 1 fps, then subsampled to ensure that no more than 64 frames are processed per video.  
We adopt top\_p = 0.001 and temperature = 0.01 to achieve greedy decoding. Flash Attention 2 \citep{dao2023flashattention} is used as the efficient attention operator. All benchmark evaluations are performed on NVIDIA A6000 GPUs with 48GB of memory. Appendix A includes more details.
Our baseline experiments are conducted using Qwen2.5-VL-3B~\citep{bai2025qwen2}.  
We further evaluate on several widely used small-scale vLLMs, including Gemma3~\citep{team2025gemma}, InternVL-3.5-2B, and InternVL-3.5-4B~\citep{wang2025internvl3}. 
In addition, we compare our approach against representative training-free token compression strategies, namely ByteVideoLLM~\citep{wang2024dynamic}, MovieChat~\citep{song2024moviechat}, and VidCom~\citep{liu2025video}. We reproduce their methods on Qwen2.5-VL-3B. For temporal compression methods (e.g., MovieChat), inputs are compressed to a single frame, yielding the same effective input length as our method.  
For spatial or mixed compression methods (e.g., VidCom and ByteVideoLLM), we ensure that the average number of vision tokens is approximately 120, equivalent to the number in our method. Only the MARC-3B experiments employ VMR for benchmark processing, with top-$k=3$. Further implementation details are included in Appendix~A.  




\textbf{Training data.}  
For training, we utilize the Video-R1-260K dataset~\citep{feng2025video}, which is sampled from a variety of public datasets. We only randomly sampled 5K instances from this dataset, consisting of videos and images, for C-GRPO training. While the image data will not contribute to compression reward, it serves to help models develop generalized reasoning abilities in static contexts~\citep{feng2025video}. The data distribution is listed in Figure~\ref{fig:training_dataset}. Appendix B contains more details regarding the training data.



\begin{table*}[t]
% \caption{Performance of different models on benchmarks.}
    \resizebox{\linewidth}{!}{%
    \setlength{\tabcolsep}{0.8mm}
     \renewcommand\arraystretch{1.3}
\begin{tabular}{@{}ccccc|cccc@{}} % <- added one 'c' at the end for the new column
\toprule
\multirow{4}{*}{Models}              & \multirow{4}{*}{Frames} & \multicolumn{3}{c}{\multirow{2}{*}{Video Reasoning Benchmark}}                          & \multicolumn{3}{c}{\multirow{2}{*}{Video General Benchmark}}                                  &  \\ 
                                     &                         & \multicolumn{3}{c}{}                                                                    & \multicolumn{3}{c}{}                                                                          &  \\ \cmidrule(l){3-8} 
                                     &                         & \multirow{2}{*}{\small VSI-Bench} & \multirow{2}{*}{\small VideoMMMU} & \multirow{2}{*}{\small MMVU (mc)} & \multirow{2}{*}{\small MVBench} & \multirow{2}{*}{\small TempCompass} & \multirow{2}{*}{\small VideoMME (w/o sub)} & \multirow{2}{*}{\small mean} \\
                                     &                         &                            &                            &                               &                          &                              &                                     &  \\ \midrule %\rowcolor{Gray}
Qwen2.5-VL-3B~\citep{bai2025qwen2} & 64 & 32.93 & 35.33 & 48.64 & 44.77 & 38.05  & 53.55& 42.21\\ %\rowcolor{Gray} 
Qwen2.5-VL-3B~\citep{bai2025qwen2} & 16 & 27.63 & 30.78 & 45.28 & 43.89 & 37.95  & 44.37 & 38.32\\  
InternVL3.5-2B~\citep{wang2025internvl3} & 64 & 14.65 & 15.56 & 22.88 & 14.71 & 23.63 & 4.26 & 15.95 \\
InternVL3.5-4B~\citep{wang2025internvl3} & 64 & 28.96 & 33.33 & 47.51 & 44.71 & 58.34 & 39.15 & 42.00 \\
Gemma-3-4B~\citep{team2025gemma} & 64 & 26.83 & 26.78  & 41.76 & 36.82 & 55.04 & 46 & 38.87\\
\midrule
ByteVideoLLM-3B~\citep{wang2024dynamic} & 64 & 21.33  & 22.33 & 28.63 & 22.56 & 35.55 & 22.7& 25.52\\  
MovieChat-3B~\citep{song2024moviechat} & 1 & 25.14 & 25.78  & 39.35 & 37.1 & 38.79 & 26.41 & 32.10\\
VidCom\(^2\)-3B~\citep{liu2025video} & 64 & 25.5 & 23.89  & 31.08 & 29.88 &35.23 & 21.48 & 27.84\\
\midrule
\textbf{MARC-3B}  & \textbf{1} & \textbf{27.55} & \textbf{33.11}& \textbf{51.99} & \textbf{45.82} & \textbf{55.34} & \textbf{39.44}& \textbf{42.20}\\
\bottomrule

\end{tabular}
}

\caption{\textbf{Performance of different models/methods on benchmarks.} We evaluated three models (Qwen2.5-VL, InternVL3.5, and Gemma-3) and three compression methods (ByteVideoLLM, MovieChat, and VidCom\(^2\)) using a unified set of parameters. All models and methods employ 1fps sampling, but the maximum frame rate is capped (as indicated in the frame column). \textit{Note: 
% \textcolor{blue}{
The "Frame" column indicates the number of visual tokens comparable to how many frames's token that are fed into the LLM decoder before generation, not the raw video sampling rate.
% }
}}
\vspace{-5mm}
\label{tab:main_table}
\end{table*}







\begin{figure*}[t]
    \centering
    \begin{minipage}{0.42\linewidth} 
        \centering
        \includegraphics[width=\linewidth]{figures/evaluation_dataset.pdf}
        \caption{Distribution of benchmarks based on the number of QA samples.}
        \label{fig:evaluation_dataset}
    \end{minipage}
    % \hfill
    \hspace{2mm} % Reduce horizontal space
    \begin{minipage}{0.42\linewidth} 
        \centering
        \includegraphics[width=\linewidth]{figures/training_data.pdf}
        \caption{Distribution of training dataset based on number of QA samples.}
        \label{fig:training_dataset}
    \end{minipage}
    \vspace{-8mm}
\end{figure*}



\textbf{Training details}. 
We adopt Qwen2.5-VL-3B as the backbone model for training. The training dataset is first pre-processed using the Visual Memory Retriever.
% All experiments are conducted on four NVIDIA H100 GPUs. 
During C-GRPO training, the full-frame teacher model processes videos with 64 frames, while the student model operates on the compressed single-frame input. The ordered group size $G$ is set to 8. Additional implementation details are provided in Appendix~B.  

\subsection{Main Comparison}
\label{sec:main_comparison}
\vspace{-4mm}
\textbf{Performance Comparison.} 
Table~\ref{tab:main_table} presents the results on six benchmarks, 
covering both video reasoning and general video understanding tasks. 
Before compression, the mean number of visual tokens per sample across all benchmarks (64 frames) is \textbf{2589.93}. 
After compression, this number is reduced to \textbf{122.69} tokens (a 95$\%$ reduction). 
Our method demonstrates competitive performance across all benchmarks 
compared with the baselines. Specifically, relative to the Qwen2.5-VL-3B baseline (64 frames), our model achieves nearly identical mean performance (42.20 vs.\ 42.21) 
while using only \textbf{4.71\%} of the visual tokens, as shown in Figure~\ref{fig:statistics}.

    
\begin{minipage}[t]{0.4\textwidth}
    \vspace{0pt}
Notably, the average score of MARC-3B also surpasses that of larger models such as InternVL3.5-4B and Gemma-3-4B.
Among the six benchmarks, our method outperforms the Qwen2.5-VL-3B baseline on MMVU, MVBench, and TempCompass. The substantial improvement on TempCompass can be attributed to the enhanced instruction-following ability obtained through our training process, which effectively addresses the weakness of small-scale (3B) models.
\end{minipage}%
\hfill
\begin{minipage}[t]{0.58\textwidth}
    \raggedleft
    \vspace{0pt}
    \includegraphics[width=1\linewidth]{figures/MARC.pdf}
    \captionof{figure}{Vision tokens for each benchmark and MARC compared with the baseline performance.}
    \label{fig:statistics}
\end{minipage}




For long video evaluation on VideoMME, our model inevitably incurs some performance loss due to extreme compression, retaining \textbf{74\%} of the baseline performance while processing only \textbf{3.21\%} of the original visual tokens. Nevertheless, even under this challenging setting, our approach still outperforms larger models such as InternVL3.5-4B, underscoring the effectiveness of C-GRPO in balancing efficiency and accuracy. Extensive analysis of this can be found in Appendix~\ref{sec:failure}.  

Our method substantially outperforms prior compression strategies. Compared to DynamicVLM, MovieChat, and VidCom, our approach improves mean accuracy by \textbf{65\%}, \textbf{31\%}, and \textbf{52\%}, respectively. MovieChat also employs short-term memory for temporal compression, and performs best among these methods, achieving results close to ours on VSI-Bench; however, it lags significantly on the other five benchmarks. VidCom adopts a selective token retention strategy, which has a similar effect to VMR, but still falls short of our model. These results indicate that naive compression strategies suffer from performance degradation under aggressive compression ratios.


\textbf{Efficiency Comparison.}
Figure~\ref{fig:efficiency} reports the real-world inference efficiency of different compression strategies. We evaluate GPU peak memory usage and inference latency on MMVU multiple-choice samples using a single NVIDIA A6000 GPU. To ensure robustness of the comparison, we fix the inference prompt and set the maximum output length to generate only the answer. More details are included in Appendix A. With a batch size of 15, the baseline Qwen2.5-VL with 64 frames occupies 41.63 GB out of 48 GB of GPU memory. When applying our compression framework, the memory usage is reduced to 11.48 GB, corresponding to a \textbf{72.4\%} reduction. 
\vspace{-0.4cm}
\begin{figure}[H]
\centering
\begin{minipage}[t]{0.48\textwidth}
    \vspace{0pt}
In terms of latency, input compression substantially reduces the number of tokens required during LLM generation, resulting in a \textbf{23.9\%} reduction in generation latency. This improvement leads to a \textbf{15.9\%} reduction in overall model generation latency. Consequently, the end-to-end latency for processing a single MMVU sample is reduced by \textbf{11.1\%}. These results confirm that our method achieves substantial improvements in memory efficiency and inference speed, enabling faster and more resource-efficient deployment of vLLMs in practice. 
\end{minipage}%
\hfill
\begin{minipage}[t]{0.48\textwidth}
    \raggedleft
    \vspace{0pt}
    \includegraphics[width=\linewidth]{figures/efficiency.pdf}
    \caption{Efficiency Comparison: We compared GPU memory usage and LLM generation rates.}
    \label{fig:efficiency}
\end{minipage}
\end{figure}





\subsection{Ablation studies}
\label{sec:ablation_studies}
\textbf{In comparison to training-based compression using SFT.} To evaluate the overall effectiveness of our framework, we first train a model using standard SFT on 10K samples from Video-R1-COT-165K~\citep{feng2025video}, and evaluate it on the same benchmarks (implementation details are provided in Appendix~B). Table~\ref{ablation_1} shows the result. Comparing MARC-3B-0.6 with this SFT baseline, we observe consistent improvements across all benchmarks. In terms of mean performance, our model achieves 42.20 compared to 38.50, yielding a relative gain of \textbf{+9.6\%}.
Furthermore, even against a stronger SFT+VMR variant, our method still delivers higher scores across all benchmarks (increasing mean score by 5$\%$. These results demonstrate that the integration of C-GRPO with VMR is crucial for boosting performance under extreme temporal compression.


\begin{table*}[t!]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccccccc}
\toprule
Models & Frames & \small VSI-Bench & \small VideoMMMU & \small MMVU (mc) & \small MVBench & \small TempCompass & \small VideoMME (w/o sub) & \small mean \\
\midrule
Qwen2.5-VL-3B(baseline) & 64 & 32.93 & 35.33 & 48.64 & 44.77 & 38.05 & 53.55& 42.21\\
Qwen2.5-VL-3B(VMR) & 64 & 34.02  & 34.33 & 55.52 & 57.24 &40.38 & 51.85& 45.56\\
Qwen2.5-VL-3B(SFT+VMR) & 1 & 26.71 & 31.00& 47.83& 43.91&53.76 &37.77&40.16\\ 
Qwen2.5-VL-3B(SFT) & 1 & 25.70 & 28.33 & 45.76& 39.48 & 54.05 & 37.72 & 38.50\\ 

\textbf{MARC-3B-0.6(VMR)}  & 1 & 27.55 & 33.11& 51.99 & 45.82 & 55.34 & 39.44& 42.20\\
\bottomrule
\end{tabular}}
\caption{Comparative experiments evaluating the effect of the Visual Memory Retriever (VMR) and contrasting our proposed MARC distillation framework with conventional supervised fine-tuning.}
\label{ablation_1}
\vspace{-3mm}
\end{table*}





\textbf{Ablation studies on the effect of $\tau$ in C-GRPO.} 
Table~\ref{tab:cgrpo_tao} presents the ablation study results for different threshold values $\tau$ during C-GRPO training. 
Recall from Equation~\ref{eq:compression_reward} that $\tau$ specifies the minimum acceptable retention ratio relative to the teacher model’s performance. 
We evaluate three values of $\tau$ (0.4, 0.6, and 0.8) using the same benchmarks and experimental setup described in Section~\ref{sec:experiments_settings}. 
We observe that setting $\tau=0.6$ achieves the best overall performance, with a mean score of 42.20 across six benchmarks. 
A lower threshold ($\tau=0.4$) makes the reward constraint too lenient, resulting in insufficient incentive to retain the teacher model's full performance. 
Conversely, a higher threshold ($\tau=0.8$) imposes an overly strict constraint, triggering the additional compression reward less frequently. 
This limits effective learning signals, restricts divergence from the baseline, and slightly reduces performance. 
These results suggest that a moderate $\tau$ strikes the right balance: it provides sufficient incentive for the model to preserve performance under compression while avoiding the overly conservative behaviour induced by stricter constraints.





\begin{table*}[t!]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccccccc}
\toprule
Models & $\tau$ & Frames & \small VSI-Bench & \small VideoMMMU & \small MMVU (mc) & \small MVBench & \small TempCompass & \small VideoMME (w/o sub) & \small mean \\
\midrule
\textbf{MARC-3B} & 0.4 & 1 & 28.27 & 31.66 & 49.12 & 45.21 & 54.72 & 39.07 & 41.34 \\
\textbf{MARC-3B} & 0.6 & 1 & 27.55 & 33.11 & 51.99 & 45.82 & 55.34 & 39.44 & 42.20 \\
\textbf{MARC-3B} & 0.8 & 1 & 28.23 & 31.78 & 49.34 & 45.89 & 54.12 & 39.03 & 41.40 \\
\bottomrule
\end{tabular}}
\caption{Ablation study results of MARC-3B with different $\tau$.}
\label{tab:cgrpo_tao}
\vspace{-0.6cm}
\end{table*}



\textbf{Ablation studies on VMR's effectiveness.}
First, we conduct an experiment using Qwen2.5-VL-3B model without training and compression, and evaluate it with VMR benchmarks (top-$k=3$). The result is shown in Table~\ref{ablation_1}. It achieves a mean score of 45.56, compared to 42.21 for the baseline, demonstrating that the VMR could boost performance. For MVBench, the increase is as high as 27.85$\%$. This is because, for videos with many clips, instead of sampling uniformly for 64 frames, we only sample in the top 3 important clips; therefore, more important frames are kept during evaluation. This could further explain MARC's effectiveness. It combines both the effect of VMR and C-GRPO, so that the model's reasoning ability rises, and we kept more important frames before compression. This combination achieves optimal performance. 
The effectiveness is further established by the result between SFT+VMR and SFT, we can see that the mean score increases by 4.3$\%$. For VideoMMU and MVBench, this increase reaches more than 10$\%$.

%if needed, could add a VMR+videocommander or dynamic, This also leaves the insight that other compression methods could also use VMR





==> iclr2026/framework.tex <==
\begin{figure}[t!]
    \centering
        \includegraphics[width=0.9\textwidth]{C-GRPO.pdf}
\caption{
% \textcolor{blue}{
\textbf{Left:} Visual Memory Compression. We processed the original video using two approaches: (1) Employing a visual memory retriever to search the video, subsequently reconstructing a new video and compressing its visual features; (2) Also employing a visual memory retriever to search the video, then sampling the original video before feeding it into a visual encoder to obtain uncompressed visual features. \textbf{Right:} Compression Group Relative Policy Optimization (C-GRPO) Distillation Framework. Here, \textbf{O} denotes the outputs from different groups, \textbf{R} the corresponding rewards, and \textbf{A} the normalized advantages. A compression reward $r_c$ is introduced to encourage compressed inputs to retain the reasoning ability of the uncompressed teacher model.
}
% }
    \label{fig:pipeline}
\end{figure}

==> iclr2026/framework2.tex <==
\begin{figure}[t!]
    \centering
        \includegraphics[width=0.9\textwidth]{iclr2026/framework_stage2.pdf}
\caption{\textbf{Overview of Compression Group Relative Policy Optimization (C-GRPO)}. 
Here, \textbf{O} denotes the outputs from different groups, \textbf{R} the corresponding rewards, and \textbf{A} the normalized advantages. 
A compression reward $r_c$ is introduced to encourage compressed inputs to retain the reasoning ability of the uncompressed teacher model.}
    \label{fig:pipeline2}
\end{figure}

==> iclr2026/introduction.tex <==
\section{Introduction}
\label{sec:introduction}

Recent advances in large language models (LLMs) have enabled visual language models (VLMs) to reason over multimodal inputs that combine text and images~\citep{liu2023visual,zhu2025internvl3,bai2025qwen2}. Although early applications primarily targeted short context image tasks, the demand for long context video understanding has dramatically increased computational costs. A single image may necessitate thousands of tokens; this computational load is further magnified when extending the model to high frame rate, long-duration video content. This overhead introduces significant latency and memory bottlenecks, hindering the deployment of VLMs in latency-sensitive and resource-constrained applications such as autonomous driving and surveillance systems. To mitigate these challenges, token compression techniques have been explored, with training-free visual token compression as one of the most effective strategies~\citep{li2025tokenpacker,yang2025visionzip,zhang2024sparsevlm}. Despite the fact that these methods reduce computational overhead, their training-free approach inherently causes a considerable amount of information loss during token compression, leading to a significant drop in performance.

To overcome these challenges, we propose \textbf{MARC}, a \underline{M}emory-\underline{A}ugmented \underline{R}L Token \underline{C}ompression method for efficient video understanding. Our approach is a \textbf{ retrieve and then compress} method, which first uses a \textbf{ visual memory retriever (VMR)} to identify the most relevant event segments from a video. Following this, we introduce a novel deep compression technique, \textbf{Compression Group Relative Policy Optimization (C-GRPO)}, to further compress these retrieved visual memories. This enables us to reduce each video to a token count equivalent to that of a single image while maintaining performance comparable to the uncompressed video.

Specifically, the design of our \textbf{Visual Memory Retriever (VMR)} was inspired by insights from cognitive science and neuroimaging. 
Most existing methods handle temporal and spatial redundancy independently~\citep{wang2024dynamic,liu2025video,song2024moviechat}, overlooking the temporally organized and context-aware characteristics of human visual memory. Cognitive science suggests that humans segment continuous experiences into discrete events and recall them through episodic memory, reinstating both low and high-level perceptual features~\citep{james1890principles,hebb1968concerning,damasio1989time,mcclelland1995there}. Neuroimaging studies further show reengagement of visual cortical regions during memory retrieval~\citep{favila2022perception}, while event segmentation theory emphasises contextual shifts as natural anchors for recall~\citep{li2025hierarchical}. Motivated by these principles, we propose a Visual Memory Retriever that partitions videos into semantically coherent event-level segments and retrieves query-relevant fragments. These fragments are rearranged and sampled, functioning as structured “episodic memories” for downstream reasoning and enabling more human-like temporal processing. By adopting this retrieve-then-compress approach, it dramatically reduces the computational burden and mitigates the negative effects of redundant information on compression quality.

 
To reduce a video’s token count to that of a single frame while ensuring maximum performance after compression, we proposed a post-training compression algorithm based on reinforcement learning, \textbf{Compression Group Relative Policy Optimization (C-GRPO)}, which is applied after finding the most relevant memory fragments. The traditional GRPO~\citep{shao2024deepseekmath} algorithm is used to enhance the model's reasoning capabilities. We have customized and improved its training framework, reward design, and training strategy, and for the first time, propose C-GRPO. This allows the Student Network to retain Teacher-level reasoning ability under aggressive compression, ensuring robustness while drastically lowering computational cost. Specifically, our C-GRPO transfers reasoning ability from a Teacher Network with 64 frames as input, to the Student Network with just one frame’s worth of tokens as input. 
By integrating structured retrieval with RL-based compression, our framework bridges efficiency and accuracy, providing both cognitive grounding and practical scalability.


We conduct extensive experiments across six benchmarks covering both video reasoning and general video understanding. Our framework achieves nearly identical mean performance to the 64-frame Qwen2.5-VL-3B baseline (42.20 vs.\ 42.21) while using only a single frame, corresponding to just 4.71\% of the original visual tokens. Ablation studies further validate the role of each component: Visual Memory Retriever alone boosts baseline accuracy, while C-GRPO ensures stable performance retention under extreme compression. Combined, they yield superior results, with substantial gains on challenging benchmarks such as TempCompass and MVBench. Moreover, efficiency evaluations demonstrate a 72\% reduction in GPU memory usage and 23.9\% lower generation latency, enabling deployment in real-world scenarios with strict resource constraints. 

In summary, our contributions are threefold:
\begin{itemize}
    \item We propose \textbf{MARC}, a novel framework for efficient video understanding. By deftly integrating a structured visual retrieval mechanism with a powerful reinforcement learning based token compression algorithm, our approach achieves exceptional efficiency while preserving high performance.  
    % We propose a \textbf{Visual Memory Retriever} that segments videos into event-level fragments and selects QA-relevant segments, enabling structured and efficient temporal compression.
    \item We propose \textbf{Compression Group Relative Policy Optimization (C-GRPO)}, the first post-training reinforcement learning (RL) strategy specifically designed for video token compression. C-GRPO transfers the complex reasoning ability from a high token "Teacher" network to a low token "Student" network. 
    % We introduce \textbf{C-GRPO}, a reinforcement learning-based distillation strategy that compresses 1 fps inputs into a single frame while preserving teacher-level reasoning performance.
    \item Our extensive experiments across six benchmarks demonstrate that MARC achieves both superior performance and exceptional efficiency. By reducing \textbf{GPU memory usage by 72\%} and cutting \textbf{generation latency by 23.9\%}, our approach maintains performance while enabling deployment in resource-constrained applications.
    % We demonstrate through extensive experiments that our framework achieves performance comparable to 64-frame baselines while reducing memory usage and inference latency, offering a lightweight yet effective solution for practical video understanding in edge and resource-constrained environments.
\end{itemize}

==> iclr2026/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> iclr2026/methods.tex <==
\section{Memory-Augmented RL Distillation}
\label{sec:methods2}

\subsection{Visual Memory Retriever}

\label{sec:methods}
The core principle of the Visual Memory Retriever is to prioritize the retrieval of the most task-relevant video segments before subsequent compression. This \textbf{retrieve then compress} strategy significantly reduces the computational burden while effectively eliminating the negative impact of redundant information on compression quality. This retriever is engineered to transform a continuous video stream into a structured, searchable memory bank, enabling efficient retrieval of relevant visual information to support complex downstream tasks such as video based question answering. 

\subsubsection{Event-Based Video Segmentation}
\label{subsec:segmentation}
Unlike conventional methods that rely on fixed length temporal windows, our approach employs an event based video segmentation module~\citep{soucek2024transnet} to partition long videos into semantically coherent short clips. This module leverages a deep event detection network that analyzes the video stream to identify significant temporal boundaries, such as scene changes, topic shifts, or the commencement of new actions. Each resulting clip, or visual memory fragment, encapsulates a complete and meaningful event, thereby preserving the contextual integrity of the original video. This event-centric approach dramatically reduces the search space for subsequent retrieval steps and ensures that each retrieved fragment is a complete and self contained unit of information.

\subsubsection{Memory Retrieval}
\label{subsec:retrieval}
The next stage is the retrieval of memory. We map both the inferred query representation and the visual memory fragments into a shared, high-dimensional latent space using an embedding model~\citep{bolya2025perception}. This space is learned using a contrastive learning framework, ensuring that semantically similar query fragment pairs are located in close proximity. 
The search process is performed across the entire corpus of visual memory fragments that are semantically related to the query. This step utilizes a highly optimized nearest neighbor search algorithm on the pre-indexed fragment embeddings, allowing for efficient filtering. The final output is an ordered list of the top-$k$ visual memory fragments, which are then passed to a downstream compression model. This retriever provides the LLM with the precise visual evidence required to ground its response, thereby mitigating hallucination and enabling true video-based reasoning.

==> iclr2026/methods_2.tex <==


\input{framework}

% \subsection{Compression Layer}

% We adopt a commonly used cosine similarity-based token merging approach for temporal compression, following prior work such as MovieChat~\citep{song2024moviechat}. As described in Section~\ref{sec:methods}, we first obtain $k$ segments from the \textbf{Visual Memory Retriever}. As shown in Figure~\ref{fig:pipeline}, these $k$ segments are then rearranged and sampled at 1 fps to obtain $N$ frames. Concretely, given an input video with $N$ frames, each frame is encoded by a visual encoder (e.g., ViT) into patch-level hidden states. Let  
% \begin{equation}
% \mathcal{H} = \{\mathbf{h}_1, \mathbf{h}_2, \dots, \mathbf{h}_T\}, \quad \mathbf{h}_i \in \mathbb{R}^{d},
% \label{eq:H_tokens}
% \end{equation}  
% denote the sequence of $T$ visual tokens, where $T = N \cdot P$ and $P$ is the number of patches per frame. We partition $\mathcal{H}$ along the temporal dimension into short-term memory segments of length $m$ frames:  
% \begin{equation}
% \mathcal{S}_j = \{\mathbf{H}_{(j-1)m+1}, \dots, \mathbf{H}_{jm}\}, \quad j = 1, \dots, \left\lceil \tfrac{N}{m} \right\rceil,
% \label{eq:segment_partition}
% \end{equation}  
% where each $\mathbf{H}_t \in \mathbb{R}^{P \times d}$ represents the $P$ visual tokens from frame $t$. Within each segment $\mathcal{S}_j$, we iteratively merge the two most similar consecutive frame-level embeddings $\mathbf{H}_a$ and $\mathbf{H}_b$, where similarity is measured by cosine similarity between their token sets:  
% \begin{equation}
% \text{sim}(\mathbf{H}_a, \mathbf{H}_b) = \frac{1}{P}\sum_{p=1}^{P} \frac{\mathbf{h}_a^{(p)} \cdot \mathbf{h}_b^{(p)}}{\|\mathbf{h}_a^{(p)}\|\|\mathbf{h}_b^{(p)}\|}.
% \label{eq:cosine_similarity}
% \end{equation}  
% The merging replaces them with their mean:  
% \begin{equation}
% \mathbf{H}_{\text{merge}} = \tfrac{1}{2}\,(\mathbf{H}_a + \mathbf{H}_b).
% \label{eq:merge_mean}
% \end{equation}  
% This process continues until the retained number of frames in $\mathcal{S}_j$ reaches  
% \begin{equation}
% n_j = \max\!\left(1, \left\lfloor (1-\rho)\cdot |\mathcal{S}_j| \right\rfloor \right),
% \label{eq:retain_frames}
% \end{equation}  
% where $\rho \in (0,1)$ is the compression ratio. After segment-wise compression, all segments are concatenated into $\mathcal{H}' = \{\mathbf{H}'_1, \dots, \mathbf{H}'_{N'}\}$. If $N' > N_{\text{target}} = \lfloor (1-\rho)N \rfloor$, we further perform cross-segment merging with the same averaging rule until $N' \leq N_{\text{target}}$. The resulting compressed sequence $\mathcal{H}'$ thus consists of temporally compressed visual tokens, along with the updated grid structure $\text{THW}'$, which are then passed into the subsequent transformer layers.

% \subsection{Compression Group Relative Policy Optimization (C-GRPO)}
% \input{iclr2026/framework2}

% We formulate compression learning as a distillation process in which the reasoning capability of a full-frame teacher (64 frames) is transferred to a single-frame student representation. While standard GRPO~\citep{shao2024deepseekmath} enforces output correctness and format consistency, it does not ensure that compressed inputs preserve the performance of their full-frame counterparts. As shown in Figure~\ref{fig:pipeline2}, to address this limitation, we propose \textbf{Compression Group Relative Policy Optimization (C-GRPO)}, which introduces an auxiliary reward explicitly aligning compressed performance with the teacher baseline.  

% Let $a_{\text{full}}$ represent the average reward obtained using the 64-frame input and $a_{\text{comp}}$ denote the reward under the compressed one-token input. We define the \emph{retention ratio}:  
% \begin{equation}
% \eta = \frac{a_{\text{comp}}}{a_{\text{full}}},
% \label{eq:retention_ratio}
% \end{equation}  
% which measures how effectively the compressed input retains the teacher’s performance. Based on this, we introduce a \emph{compression reward}:  
% \begin{equation}
% r_c = \alpha \cdot \max(0,\; \eta - \tau),
% \label{eq:compression_reward}
% \end{equation}  
% where $\tau = 0.6$ specifies the minimal acceptable fraction of teacher performance, and $\alpha$ controls the strength of the additional reward. The total reward for each sample is then:  
% \begin{equation}
% R_i = r_i + \mathbbm{1}[\text{correct}]\, r_c,
% \label{eq:total_reward}
% \end{equation}  
% with $r_i$ as the base GRPO reward. Only correct responses receive the compression reward, ensuring stable and reliable learning signals.  

% The advantage for each sample is normalised as:  
% \begin{equation}
% A_i = \frac{R_i - \bar{R}}{\sigma_R},
% \label{eq:advantage}
% \end{equation}  
% where $\bar{R}$ and $\sigma_R$ denote the batch mean and standard deviation of rewards, respectively. Finally, the optimisation objective is:  
% \begin{equation}
% \mathcal{L}_{\text{C-GRPO}} = 
% \mathbb{E}\!\left[
%   \frac{1}{G}\sum_{i=1}^G 
%   \Big(
%     \text{clip}\!\left(
%       \frac{\pi_\theta(o_i \mid q)}{\pi_{\theta_{\text{old}}}(o_i \mid q)},\; 1-\epsilon,\; 1+\epsilon
%     \right) 
%     A_i 
%   \Big)
%   - \beta\, \mathrm{KL}\bigl(\pi_\theta \,\|\, \pi_{\text{ref}}\bigr)
% \right].
% \label{eq:cgrpo_loss}
% \end{equation}  

% This formulation allows C-GRPO to act as a distillation mechanism that encourages compressed representations to approximate full-frame performance, achieving efficient yet effective reasoning under aggressive temporal compression.





\subsection{RL-based Video Token Compression}

Building on the {Visual Memory Retriever (VMR)} in Section~\ref{sec:methods}, which transforms long videos into a small set of query-relevant, event-level segments, we first introduce a memory-aware temporal compression layer that is tailored to these retrieved segments. Then, we propose the Compression Group Relative Policy Optimization to maintain performance despite extreme token compression.

\subsubsection{Memory-Aware Temporal Compression Layer}
\label{sec:compression}
Rather than treating compression as a generic, training-free pre-processing step, our design exploits the structure imposed by VMR: we first preserve short-range temporal coherence inside each retrieved segment, then perform cross-segment consolidation. This memory-first strategy ensures that compression removes redundancy where it is most prevalent (nearby frames within the same episode) while keeping the event evidence that VMR deemed relevant for downstream reasoning. Concretely, we extend cosine similarity based frame merging (in the spirit of prior temporal ToMe methods such as MovieChat~\citep{song2024moviechat}) into a two stage, memory aware procedure that (i) merges highly similar consecutive frames inside each short-term segment to retain local dynamics and (ii) applies a global, light weight consolidation only when the token budget still exceeds the target. This coupling to VMR is key: the compressor is not a standalone heuristic but an intent-aligned module that respects the event boundaries and ranking produced by VMR, thereby preserving the most causally useful frames for QA.

As shown in Figure~\ref{fig:pipeline}, we first obtain $k$ top-ranked segments from VMR and uniformly sample them at 1 fps to obtain $N$ frames. Each frame is encoded by a visual encoder (e.g., ViT) into patch-level hidden states. Let
\begin{equation}
\mathcal{H} = \{\mathbf{h}_1, \mathbf{h}_2, \dots, \mathbf{h}_T\}, \quad \mathbf{h}_i \in \mathbb{R}^{d},
\label{eq:H_tokens}
\end{equation}
denote the sequence of $T$ visual tokens, where $T = N \cdot P$ and $P$ is the number of patches per frame. We then partition $\mathcal{H}$ along the temporal axis into short-term memory windows of length $m$ frames (intuitively, contiguous frames within one episode); the $j$-th window contains frames indexed from $(j\!-\!1)m+1$ to $jm$ (inclusive):
\begin{equation}
\mathcal{S}_j = \{\mathbf{H}_{(j-1)m+1}, \dots, \mathbf{H}_{jm}\}, \quad j = 1, \dots, \left\lceil \tfrac{N}{m} \right\rceil,
\label{eq:segment_partition}
\end{equation}
where each $\mathbf{H}_t \in \mathbb{R}^{P \times d}$ stacks the $P$ patch tokens of frame $t$. Inside each $\mathcal{S}_j$ we iteratively merge the two most similar consecutive frame embeddings $\mathbf{H}_a$ and $\mathbf{H}_b$ (consecutive in time), where similarity averages patch-aligned cosine scores (the ViT grid provides a natural patch correspondence):
\begin{equation}
\text{sim}(\mathbf{H}_a, \mathbf{H}_b) = \frac{1}{P}\sum_{p=1}^{P} \frac{\mathbf{h}_a^{(p)} \cdot \mathbf{h}_b^{(p)}}{\|\mathbf{h}_a^{(p)}\|\|\mathbf{h}_b^{(p)}\|}.
\label{eq:cosine_similarity}
\end{equation}
The two frames are replaced by their mean representation,
\begin{equation}
\mathbf{H}_{\text{merge}} = \tfrac{1}{2}\,(\mathbf{H}_a + \mathbf{H}_b),
\label{eq:merge_mean}
\end{equation}
and this process repeats until the retained frames in $\mathcal{S}_j$ reach the budget
\begin{equation}
n_j = \max\!\left(1, \left\lfloor (1-\rho)\cdot |\mathcal{S}_j| \right\rfloor \right),
\label{eq:retain_frames}
\end{equation}
where $\rho \in (0,1)$ is the overall compression ratio (smaller $\rho$ keeps more frames). Finally, we concatenate all compressed segments into $\mathcal{H}' = \{\mathbf{H}'_1, \dots, \mathbf{H}'_{N'}\}$; if $N' > N_{\text{target}} = \lfloor (1-\rho)N \rfloor$, we perform a light cross segment merge (same averaging rule) so that local episode structure is preserved first and global pruning acts only as a last resort. The resulting $\mathcal{H}'$ is thus a temporally compressed, memory aware token sequence (with updated grid $\text{THW}'$) that is well aligned with the VMR selected evidence and ready for subsequent transformer layers.

\subsubsection{Compression Group Relative Policy Optimization (C-GRPO)}
% \input{iclr2026/framework2}

We formulate the compression process as a distillation problem: a full-frame teacher provides the reference behaviour, while a single-frame student learns to match its reasoning quality under an aggressively reduced token budget. Standard GRPO~\citep{shao2024deepseekmath} enforces answer correctness and format but does not explicitly couple student performance to its full-frame counterpart; in contrast, our \textbf{C-GRPO} adds a retention alignment reward that directly encourages compressed inputs to preserve teacher-level performance, as illustrated in Figure~\ref{fig:pipeline}. Formally, let $a_{\text{full}}$ be the average reward with 64 frame inputs and $a_{\text{comp}}$ the reward with the compressed input; the retention ratio
\begin{equation}
\eta = \frac{a_{\text{comp}}}{a_{\text{full}}},
\label{eq:retention_ratio}
\end{equation}
quantifies how much of the teacher’s performance the student retains under compression. We then shape the objective with a compression reward
\begin{equation}
r_c = \alpha \cdot \max(0,\; \eta - \tau),
\label{eq:compression_reward}
\end{equation}
where $\tau$ specifies the minimum acceptable retention and $\alpha$ scales the incentive. Intuitively, $\tau$ trades off stability and ambition: too low a threshold tolerates under retention; too high makes positive signals sparse and slows learning. In practice, we set $\tau\!=\!0.6$ as a balanced choice validated by ablations (it yields the best mean across benchmarks while maintaining stable training), and we defer full sensitivity analysis to our ablation section. To avoid rewarding confidently wrong behaviours and amplifying spurious patterns, we gate this bonus by correctness:
\begin{equation}
R_i = r_i + \mathbbm{1}[\text{correct}]\, r_c,
\label{eq:total_reward}
\end{equation}
So only semantically valid generations can earn retention credit. This gating reduces reward hacking, stabilises learning signals, and focuses policy updates on trajectories that already satisfy task constraints. We normalise advantages within each group to reduce variance,
\begin{equation}
A_i = \frac{R_i - \bar{R}}{\sigma_R},
\label{eq:advantage}
\end{equation}
and optimise the clipped objective with a KL anchor to a reference policy:
\begin{equation}
\mathcal{L}_{\text{C-GRPO}} = 
\mathbb{E}\!\left[
  \frac{1}{G}\sum_{i=1}^G 
  \Big(
    \text{clip}\!\left(
      \frac{\pi_\theta(o_i \mid q)}{\pi_{\theta_{\text{old}}}(o_i \mid q)},\; 1-\epsilon,\; 1+\epsilon
    \right) 
    A_i 
  \Big)
  - \beta\, \mathrm{KL}\bigl(\pi_\theta \,\|\, \pi_{\text{ref}}\bigr)
\right].
\label{eq:cgrpo_loss}
\end{equation}
Together with the memory-aware compressor, C-GRPO turns compression into an alignment problem, retaining the teacher’s reasoning where it matters rather than a purely geometric token reduction heuristic, yielding both efficiency and robustness under extreme temporal compression.

==> iclr2026/related_works.tex <==

\section{Related Work}



\noindent\textbf{Video Compression for Large Language Models.}
Recent advances in multimodal large language models (MLLMs) have greatly expanded their applicability to a wide range of video understanding tasks~\citep{bai2025qwen2,li2024llava}. These models generally process videos by employing powerful pre-trained visual encoders such as CLIP~\citep{radford2021learning} and SigLIP~\citep{zhai2023sigmoid} to transform sampled video frames into visual tokens that can be fed into the language model. This design allows MLLMs to integrate visual and textual information effectively, enabling tasks such as video captioning, temporal reasoning, and question answering. However, when dealing with long or high-resolution videos, practical limitations such as restricted context length, GPU memory constraints, and increased computational cost create a challenging trade-off between the number of tokens per frame and the total number of frames processed. To address these challenges, prior approaches have explored compression techniques~\citep{song2024moviechat}, adaptive pruning mechanisms~\citep{wang2024dynamic}, and frame selection strategies during inference~\citep{wang2024videoagent}. While these methods can alleviate computational overhead, they often suffer from substantial performance degradation, particularly when critical temporal or spatial information is discarded. In contrast, our work proposes a novel reinforcement learning based distillation framework that substantially reduces the required number of visual tokens without sacrificing accuracy. By aligning compressed representations with the reasoning ability of a 1fps sampling teacher model, our approach results in faster inference, lower GPU memory usage, and improved efficiency for real world video understanding applications.



\noindent\textbf{Video Retrieval Augmented Generation.}
Video-RAG is a specialized branch of MM-RAG, with its core function being the utilization of video corpora for knowledge retrieval and subsequent generation \citep{lewis2020retrieval,jeong2025videorag}. Based on the primary methods for integrating videos with vLLMs, we can categorize existing Video-RAG architectures into the following: \textbf{Auxiliary Text Enhancement:} This category of methods aims to circumvent the challenges of directly processing dense video frames by converting video content into concise, query-auxiliary text \citep{wang2022language,edge2024local,pan2023retrieving}. This auxiliary text can be spoken content generated by Automatic Speech Recognition (ASR), on-screen text extracted via Optical Character Recognition (OCR), or visual descriptions produced by object detection. This "text-based" concept greatly simplifies the ingestion process and significantly reduces computational overhead, thereby making long video comprehension possible. \textbf{Corpus Retrieval:} This paradigm focuses on dynamically retrieving video clips or entire videos from a large video corpus that are relevant to a given query. These retrieved contents are then fed to a generator as a knowledge source \citep{luo2021clip4clip,ren2025videorag}. This method is particularly suited for queries that require finding specific events or information from a massive video library. \textbf{Agent-Based Systems:} These frameworks, exemplified by VideoAgent \citep{wang2024videoagent} and M3-Agent \citep{long2025seeing}, use a large language model (LLM) as a core agent to mimic a human's multi-round reasoning process. The LLM agent iteratively plans, retrieves, and refines information from the video, using tools such as Visual Language Models (VLMs) and Contrastive Language Image Pretraining (CLIP) to assist in decision-making until the question is fully answered. This approach is especially effective for long video question answering that requires complex, multi-step reasoning. In this paper, we adopt the video corpus retrieval scheme. By using efficient video segmentation and retrieval, we can effectively and significantly reduce the number of input tokens and minimize unnecessary computational overhead.




